Unsupervised 3D Learning for Shape Analysis via Multiresolution Instance Discrimination

Although unsupervised feature learning has demonstrated its advantages to reducing the workload of data labeling and network design in many fields, existing unsupervised 3D learning methods still cannot offer a generic network for various shape analysis tasks with competitive performance to supervised methods. In this paper, we propose an unsupervised method for learning a generic and efficient shape encoding network for different shape analysis tasks. The key idea of our method is to jointly encode and learn shape and point features from unlabeled 3D point clouds. For this purpose, we adapt HR-Net to octree-based convolutional neural networks for jointly encoding shape and point features with fused multiresolution subnetworks and design a simple-yet-efficient Multiresolution Instance Discrimination (MID) loss for jointly learning the shape and point features. Our network takes a 3D point cloud as input and output both shape and point features. After training, the network is concatenated with simple task-specific back-end layers and fine-tuned for different shape analysis tasks. We evaluate the efficacy and generality of our method and validate our network and loss design with a set of shape analysis tasks, including shape classification, semantic shape segmentation, as well as shape registration tasks. With simple back-ends, our network demonstrates the best performance among all unsupervised methods and achieves competitive performance to supervised methods, especially in tasks with a small labeled dataset. For fine-grained shape segmentation, our method even surpasses existing supervised methods by a large margin.

==> tables/merge-table.tex <==
\begin{table*}[h]
  \begin{minipage}{0.46\linewidth}
    \centering
    \resizebox{1\linewidth}{!}{%
        \begin{tabular}{lccc}
            \toprule
            \multirow{2}{*}{Model} & Shape            & ShapeNet       & PartNet  \\
                                   & Classification   & Segmentation   & Segementation \\
            \midrule
            Prior Art.           & 92.9\,\small (DGCNN)   & 83.7\,\small(SPLATNet)     & 47.9\,\small (PointCNN)  \\
            \midrule
            MID-FC(NoPre)        & 92.9                   & 84.2                       & 58.4  \\
            MID-FC(Finetune)     & 93.1                   & 84.8                       & 60.8     \\
            \midrule
            PointNet-FC(NoPre)      &  90.1                  & 81.9                       & 43.8\\
            PointNet-FC(Finetune)   &  90.1                  & 83.4                       & 49.4\\
            \bottomrule
        \end{tabular}
    } % resizebox
    % \vspace{-2mm}
    \caption{
        Evaluation of our network and the MID scheme. 
    }
    \label{tab:Net-MID_Valid}
  \end{minipage}\hfill
  \begin{minipage}{0.53\linewidth}
    \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lcc||lcc}
      \toprule
      Model           & Classification     & Segementation     & Model          & Classification     & Segementation     \\
      \midrule
      MID-FC          & 90.3     & 85.5     & NoAug          & 82.3     & 83.9     \\
      \cmidrule{1-3} 
      MID-1Fusion     & 89.9     & 85.3     & NoScale        & 89.2     & 84.3     \\
      MID-NoFusion    & 88.2     & 83.1     & NoTrans        & 89.7     & 85.1     \\
      U-Net           & 89.3     & 84.5     & NoRot          & 89.9     & 85.3     \\
      \midrule
      Point-Loss      & 89.5     & 85.3     & 50-Patch       & 90.1     & 84.9     \\
      Shape-Loss      & 88.9     & 83.3     & 200-Patch      & 90.0     & 85.5     \\
                      &          &          & 400-Patch      & 90.2     & 85.4     \\
      \bottomrule
    \end{tabular}
    } % resizebox
    \caption{Ablation study of different design choices.}
    
    % \vspace{-2mm}
    \label{tab:ablation}     
  \end{minipage}
  \vspace{-10pt}
  \end{table*}
